GRASP: a GReen energy Aware SDN Platform

The transition to renewable energy sources for data centers has become a popular trend in the IT industry. However, the volatility of renewable energy, such as solar and wind power, impedes the operation of green data centers. In this work, we leverage Software Defined Networking (SDN) to build GRASP, a platform that schedules job requests to distributed data centers according to the amount of green energy available at each site. GRASP can be re-configured with different scheduling algorithms to address diverse factors such as amounts of instantly available solar power, wind power and CPU load of data centers. We utilize realistic green energy datasets from National Solar Radiation Database and evaluate GRASP in the GENI testbed; in addition, we create necessary GENI artifacts to repeat our experiment. GRASP can serve as a practical platform to test various job scheduling mechanisms for distributed green data centers.

==> Makefile <==
PRJ = aggregate

# to use eps figures
DVIOPT = -P cmz -t letter -G0

all : viewpdf 

#${PRJ}.dvi : *.tex *.bib 
#	pdflatex ${PRJ}; bibtex ${PRJ}; pdflatex ${PRJ}; pdflatex ${PRJ} 
#
#${PRJ}.ps : ${PRJ}.dvi
#	dvips ${DVIOPT} -o ${PRJ}.ps ${PRJ}.dvi

#${PRJ}.pdf : ${PRJ}.ps
${PRJ}.pdf : *.tex *.bib 
	pdflatex ${PRJ}; bibtex ${PRJ}; pdflatex ${PRJ}; pdflatex ${PRJ} 
#	ps2pdf ${PRJ}.ps ${PRJ}.pdf

dvi : ${PRJ}.dvi

ps : ${PRJ}.ps

pdf : ${PRJ}.pdf

viewdvi : ${PRJ}.dvi
	xdvi ${PRJ}.dvi &

viewps : ${PRJ}.ps
	open ${PRJ}.ps &

viewpdf : ${PRJ}.pdf
	open ${PRJ}.pdf &

# to use non-eps figures.
#all : view 

#${PRJ}.pdf : *.tex 
#	pdflatex ${PRJ}; bibtex ${PRJ}; pdflatex ${PRJ}; pdflatex ${PRJ}

#pdf: ${PRJ}.pdf

#view : ${PRJ}.pdf
#	open ${PRJ}.pdf &

pack : pdf
	/bin/rm -f ../${PRJ}.tgz; tar -zcf ../${PRJ}.tgz Makefile *.tex IEEEtran.cls net.bib ${PRJ}.pdf figure 

clean:
	/bin/rm -f *.toc *.aux *.bbl *.blg *.log *.dvi *~* *.bak ${PRJ}.pdf ${PRJ}.ps

distclean:
	/bin/rm -f *.toc *.aux *.bbl *.blg *.log ${PRJ}.dvi ${PRJ}.ps ${PRJ}.pdf *~* *.bak

#cut : ${PRJ}.dvi 
#	dvips -t letter -o summary.ps -p=2 -l=2 ${PRJ}.dvi
#	ps2pdf summary.ps summary.pdf
#	/bin/rm summary.ps \
#
#	dvips -t letter -o description.ps -p=3 -l=17 ${PRJ}.dvi
#	ps2pdf description.ps description.pdf
#	/bin/rm description.ps \
#
#	dvips -t letter -o references.ps -p=18 -l=20 ${PRJ}.dvi
#	ps2pdf references.ps references.pdf
#	/bin/rm references.ps



==> aggregation.tex <==
\section{adding route aggregation to quagga}
\label{sec:aggregation}
%
%   - background: some background on quagga (the figure showing Quagga's workflow and some explanation)
%     - challenges: not just listing the three challenges, but also how we solved each of them in one or two sentences (please be specific, not vague as I mentioned above)
%     - design: a figure showing the updated workflow and some explanation of the updated workflow
%     - module implementation: explain each module's implementation in some detail
%     
The first objective of our work is to add FIB aggregation and performance monitoring to Quagga without major code changes and negative performance impact.  This ensures that we do not inadvertently change Quagga's implementation logic and that our new features do not slow down the core routing and forwarding functionality.   These considerations led to the updated Quagga system, as depicted in Figure~\ref{fig:quagga_aa}.

\begin{figure}
\begin{center}
     \includegraphics[width=2.8in]{figures/Quagga.pdf}
\caption{\label{fig:quagga_aa}Quagga Modules with FIB Aggregation}
\end{center}
\vspace{-8mm}
\end{figure}


%\subsection{Quagga Background}

\subsection{FIB Aggregation}
\label{sec:quagga_design}

In order to aggregate the FIB without changing Quagga significantly,  we keep our FIB aggregation code out of the existing Quagga code.  We add an Interception Module to intercept every FIB update after it is received by the Zebra daemon and pass them to the FIB Aggregation Module (Figure~\ref{fig:quagga_aa}).  Once the Interception Module receives the aggregated FIB changes back from the FIB Aggregation module, it applies them to the Kernel FIB.   Below we describe these two modules in detail.

The Interception Module's major functionality includes fetching static routes, interception of inbound FIB updates, application of aggregated FIB updates to the Kernel FIB, and logging.  The FIB updates fall into two categories: (a) \emph{Route Installs}: adding one or more entries from the FIB for a new address prefix; and (b) \emph{Route Uninstalls}: deleting one or more entries from the FIB for an existing address prefix.   

%TODO: need more detail on aggregation module
The Aggregation Module interacts directly with the Interception Module but not with other parts of Quagga.  It houses some temporary data structures that are needed to perform effective and incremental table aggregation.  It currently encapsulates the logic of our FIFA-S  algorithm~\cite{Liu13:FIFA} which can be easily replaced with any other FIB aggregation algorithm.   Below we highlight several implementation issues that we did not encounter in our previous stand-alone implementation.

%TODO: need better explanation of the following issues.  They are very vague.
\begin{itemize}

\item \emph{Processing Static Routes}: when we plugged in the Aggregation Module to Quagga, we found a few duplicate route prefixes with different next-hop values.  It turned out that static routes were pre-configured during Quagga's start-up. Our solution is to introduce these static routes into the aggregation module but do not aggregate them.  More specifically, we set particular flags for these routes so that they will not be aggregated with other routes. 

\item \emph{Updating Kernel FIB}: without aggregation, one route change will generate one Kernel FIB change. With aggregation, however, one route change may lead to zero or more FIB changes because we have to remove redundant routes from FIB to keep it compressed all the time.   We also learned an important fact that an update with a next-hop value change actually consists of two FIB operations -- Quagga first withdraws the prefix with the old next-hop value and then injects the same prefix with a new next-hop value. 

\item \emph{Handling Recursive Next-hop}: The FIB entries propagated inside Quagga sometimes have next-hops that are "recursive" in nature. This means the next-hop to reach a destination does not refer to a direct neighbor but to another intermediate node that lies on the path to the destination.  For example, the recursive next-hop could be the iBGP neighbor that is closest to the destination (among all the iBGP neighbors of the node), but may be several IP hops away from this router.  It is therefore necessary to look up the address of the recursive next-hop in the FIB (one or more times) until we resolve this recursive next-hop to a directly connected next-hop neighbor. We did not realize the usage of recursive next-hop in Quagga initially and had difficulty understanding why the aggregated FIB is incorrect in some cases. In fact, the Quagga route data structure includes a recursive next-hop flag to determine which data field (regular next-hop or recursive next-hop) to use for the next-hop value. Since our aggregation module originally accepts and returns only non-recursive next-hop values, we had to modify our process to handle such recursive updates.

\end{itemize}

\subsection{Performance Monitoring}

When adding FIB aggregation to a routing software, we expect the changes to result in as little CPU overhead as possible and at the same time improve other performance metrics such as memory usage.  The impact of our changes can only be quantified through low level  performance metrics captured at runtime. Some metrics pertain to the overall Quagga system performance such as CPU usage and routing process' virtual memory usage.  Other metrics are specific to FIB aggregation such as FIB entry count, FIB memory usage, and number of updates made to the FIB. 

The primary statistics captured by the Performance Monitoring module include (a) CPU and virtual memory usage of the OS, BGP daemon and Zebra daemon; (b) Kernel FIB's memory usage; (c) Kernel FIB entry count; (d) number of Route Installs and Route Uninstalls intercepted and actually performed.   Part of the module is implemented within the Zebra daemon to support capturing of statistics on Zebra's updates to the Kernel FIB.

We capture the memory and CPU utilization metrics through periodic operations on the files that the Unix kernel maintains in its proc directory. 
%CPU usages are recorded in terms of multiple clock cycle values which are periodically updated in system process files. These process files also store virtual and actual memory utilizations in appropriate memory units. 
Similarly, some metrics related to the Kernel's FIB are computed from the internal kernel file /proc/net/route which holds the Kernel's FIB.  In addition, we capture routing update statistics in terms of Route Installs and Route Uninstalls by the addition of some program variables within the Zebra daemon. All the information gathered by the monitoring application is made available through command line options and log files.

%With these new additions at each network node and the basic topology creation mechanism explained earlier, we were able to create a virtual network capable of running any combination of network protocols and routing table aggregation at every node. It was therefore possible to create a working model of a real-world network architecture and access its performance metrics at every node level for any required network configuration.



==> bg.tex <==
 \section{Our Work-VeriTable}
\label{ourwork}

%section summary/organization
In this section, we will introduce the main data sturctures used in our work first, then describe the terms and design steps of VeriTable and the algorithms. Then we will use an example to show how the verification works. Finally, we theorically prove the correctness of the algorithms. 

\subsection{Patricia Trie}
\label{trie}

Instead of using a Binary Tree (BT) to store a fowarding table, we use a PATRICIA (Practical Algorithm to Retrieve Information Coded in Alphanumeric) Trie [citation] data structure, which is based on a radix tree using a radix of two. PATRICIA Trie (PT) is a compressed binary tree and can be quickly built and  perform fast IP address prefix matching. For instance, Figure~\ref{fig:patriciatries} demonstrates the corresponding PT for FIB Table~\ref{tab:fib1} and FIB Table~\ref{tab:fib2}. The most distinguished part for a PT is that the length difference between a parent prefix and child prefix can be equal and greater than 1, but it must be 1 in a BT. As a result, as shown in the example, PTs only require 5 and 4 nodes, but BTs require 8 and 7 nodes for the two tables, respectively. The differences for small tables are not big, however, they are significant for large forwarding tables with hundreds of thousands of entries. For example, an IPv4 routing table that has 575,137 entries needs 1,620,965 nodes for a BT, but only needs 1,052,392 nodes for a PT. We have detailed comparison in terms of lookup speed in Evaluation Section~\ref{sec:evaluation}. These features enable a PT to use less space and do faster search, but results in more complicated operations in terms of node creations and deletions, e.g., what if a new node with prefix $110$ needs to be added in Figure~\ref{fig:Table1Patricia}? It turns out to be that we have to use an additional glue node to accomplish the task. There are many other complex cases, but out of the scope of this work. 

\begin{figure}[t!]
	\centering
	%\captionsetup{justification=centering, width=.6\linewidth}
	
	\subfloat[Table 1\label{fig:Table1Patricia}]{
		\includegraphics[width=0.26\textwidth]{figures/Table1Patricia}
	}
	\subfloat[Table 2\label{fig:Table2Patricia}]{
		\includegraphics[width=0.15\textwidth]{figures/Table2Patricia}
	}
	%\caption*{{\small }Round one \tab Round two steps} 
	
	%\captionsetup{justification=centering, width=.9\linewidth}
	\caption{PATRICIA Tries}
	\label{fig:patriciatries}
	\vspace{-5mm}
	
\end{figure}



\subsection{Design}
\label{design}

Our design consists of two primary tasks: Building and intializing a joint PT, and a post-order forwarding quivalence verification process.

\subsubsection{Building Joint PT}
\label{sec:jointpt}

Building a joint PT for all routing/fowarding tables. Rather than building multiple BTs for each individual table and comparing them in an one-to-one peering manner, we build an accumulated PT using all tables one upon another. When building the trie, we use a number of fields on each node to help make various decisions, the detailed information is shown in Table~\ref{tab:trienode}. At the beginning, we take the first table as input and initiate all necessary fileds to construct a PT accordingly. Afterwards, during the joining process with other tables, the nodes with the same prefixes will be merged. 

Regarding next hops, we use an integer array to store them for the same prefix which is located in the same node. The size of the array is the same as the number of tables for comparison. The next hops cannot be merged because they may be different for the same prefix in different tables and also will be used for comparisons, thus they will be placed at the correspdong $n$th element in the array, where $n$ is the index number of which FIB table to input (we assume only one next hop for each distinct prefix in an FIB table in this work), e.g., For instance, the next hop $A$ of prefix $001$ in FIB Table $2$ will be assigned as the second element in the Next Hops Array on the Node with prefix $001$. If there is not a next hop for a prefix in a particular table, the element value in the array will be initialized as $"\_"$ by default, or called $"empty"$ next hop. If there is at least one $"non$-$empty"$ next hop in the array, we mark the node $Flag$ as $1$, indicating this node contains a real prefix and next hop derived from one of the tables, we call it a $REAL$ node. Otherwise, we call it a $GLUE$ node. Algorithm~\ref{alg:patriciabuild} elaborates the detailed workflow to build a joint PT for mulitple tables. Figure~\ref{fig:initialjointtrie} shows the resultant joint PT for FIB Table~\ref{tab:fib1} and ~\ref{tab:fib2}. 

There are a few advantages for the design of a joint PT: ($a$) Many common prefixes among different tables will share the same trie node and prefix, which can considerably reduce memory consumption and computational time for new node creations; ($b$) Common prefixes and uncommon prefixes will be automatically gathered and identified after the combination; and ($c$) The design will greatly speed up subsequent comparisons of next hops between multiple tables without traversing multiple tries.  

\algnewcommand\algorithmicforeach{\textbf{for each}}
\algdef{S}[FOR]{ForEach}[1]{\algorithmicforeach\ #1\ \algorithmicdo}

\begin{algorithm}
	\caption{Building the Joint FIB $T$}\label{alg:patriciabuild}
	\begin{algorithmic}[1]
		\Procedure{$BuildJointFIB$}{$T_{1..n}$}
		\State Make Patricia trie $T$
		\State Add the head node with the prefix $0/0$. 
		\State Set the head node of $T$ to a default next hop value. %$[0, ..., 0]_{n}$.
		\ForEach {table $T_{i} \in T_{1..n}$}
		\ForEach {entry $e$ in $T_{i}$}
		\State Find a node $n$ in $T$ such as $n.prefix$ is a \par
		\hskip\algorithmicindent \hskip\algorithmicindent longest match for $e.prefix$ in $T$
		\State $n_{c} \in \{n.left, n.right, \emptyset\}$ \Comment $n$'s child node
		\If {$n.prefix = e.prefix$}
		\State $n.nexthop_{i} \gets e.nexthop$
		\Else 
		\State Generate new node $n'$
		\State $n'.prefix \gets e.prefix$
		\State $n'.nexthop_{i} \gets e.nexthop$
		\If {($n_{c}$ is at the same branch as $n'$) $\land$ \par
			\hskip\algorithmicindent \hskip\algorithmicindent
			($n'.prefix$ and $n''.prefix$ are \par
			\hskip\algorithmicindent \hskip\algorithmicindent
			non-ovelapping)}
		\State Generate a glue node $g$
		\State $n'.parent \gets g$
		\State $n_{c}.parent \gets g$
		\State $g.parent \gets n$
		\State Set $g$ as a child of $n$
		\Else { $n'.prefix$ overlaps $n_{c}.prefix$} 
		\State $n'.parent \gets n$
		\State $n_{c}.parent \gets n'$
		\State Set $n_{c}$ as a child of $n'$ 
		\State Set $n'$ as a child of $n$ 
		\EndIf
		
		\EndIf
		\EndFor
		\EndFor
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

\begin{table}[tbp]
	\centering
	\small
	\caption{Trie Node Attributes}
	\label{tab:trienode}
	\captionsetup{justification=centering}
	\begin{tabular}{| l | l | p{4cm} |}
		\hline
		Attribute  & Data Type & Description   						\\ \hline 	\hline
		Parent & Node Pointer  & Pointing to its parent node						\\ \hline
		Left child & Node Pointer   & Pointing to its left child node	if exists		\\ \hline
		Right child & Node Pointer   & Pointing to its right child node if exists		\\ \hline
		Prefix & Char Array & Binary string, e.g., $0101$, size 32 for IPv4 or 128 for IPv6
		\\ \hline
		Length & Integer & The length of this prefix, 0-32 for IPv4 or 0-128 for IPv6
		\\ \hline
		Next hops & Integer Array& Next hops of this prefix in $T_{1}...T_{n}$, size $n$ 	\\ \hline
		Node type & Integer & Indicating if a node is a $GLUE$ or $REAL$ node 	\\ \hline
		Leak flag & Integer & Indicating if a node "leaks" more routing space than its children					\\ \hline
	\end{tabular}
\end{table}


\begin{figure}
	\begin{center}
		\includegraphics[width=.6\linewidth]{figures/initialjointtrie}
		\caption{\label{fig:initialjointtrie}Joint PATRICIA Trie}
	\end{center}
	\vspace{-8mm}
\end{figure}

\subsubsection{Post-Order Equivalence Verification}
\label{sec:verification} 
After building the joint PT and initializing all necessary fields, we start the verification process, which only needs one post-order PT traveral and includes two steps to accomplish the forwarding equivalence verfication as follows:  

(A) Top-down inheriting next hops. In this step, we take advantage of a simple but very important rule: \textbf{\textit{Accoring to LPM rule, the real next hop value for a prefix that has an "empty" next hop on the joint PT should be inherited from its closest ancestor, whose next hop exists and "non-empty"}}. For example, after an LPM search using prefix $000$ in Figure~\ref{fig:initialjointtrie}, the second next hop value should return $B$, which was derived from the second next hop $B$ of its nearest ancestor-the root node. The Top-down process will help each specific prefix on a $REAL$ node in the joint PT to inherit a next hop from its closest ancestor if the prefix does have an "empty" next hop on its own. More specifically, when moving down, we compare the Next Hop array in a parent node with the Next Hop array in the child node. If there are elements in the child array with "empty" next hops, then fill them out with the same values as the parent. If there are next hops present in the child node (a $REAL$ node), then keep them. Note that all $GLUE$ nodes (hollow nodes in Figure~\ref{fig:initialjointtrie}) will be skipped during this process, because they are merely ancillary nodes helping build up the trie structure and do not carry any next hop information. After this step, every $non$-$GLUE$ node will have a new Next Hop array without any "empty" next hops. Figure~\ref{fig:topdownjointtrie} shows the results after the top-down step.

\begin{figure}
	\begin{center}
		\includegraphics[width=.6\linewidth]{figures/TopDownJointTrie}
		\caption{\label{fig:topdownjointtrie}Joint PATRICIA Trie After Top-Down Process}
	\end{center}
	\vspace{-8mm}
\end{figure}


(B) Bottom-up verify LPM next hops. In fact, this process is interweaved with the top-down process in our recursive post-order verification program. While the program moves downwards, the top-down operations will be executed. While it moves upwards, a series of operations will conducted as follows. First of all, a leaf node at the bottom may be encountered, where the Next Hop array will be checked linearly element by element. If there are any dispendancies, then we can immediately conclude that the forwarding tables yield different forwarding behaviors. In other words, they are not forwarding equivalent. If all next hops share the same value, we move upwards to its directly connected parent node, where we check the prefix length difference from the recently visited child node. Since we use PATRICIA trie as our data structure, two cases may occur: $d=1$ and $d>1$, where $d$ denotes the length difference. It is easy to infer that the child node accounts for $1/2^d$ routing space of the parent. For instance, $000$ and $001$ each accounts for $1/2$ routing space of $00$, but $100$ only accounts for $1/2^2=1/4$ routing space of $1$. The minimum value of $d$ is 1, thus one child node at most accounts for $1/2$ routing space of the parent. In other words, if $d=1$ for botn left and right child, then the two children will account for the whole routing space of the parent. The first case $d=1$ implies that the parent node does not have extra routing space to cover between itself and the child node. On the contrary, the second case $d>1$ indicates the parent node covers more routing space than that of the chidren. 

These observations are very important and inspire our verification algorithm, because correct verification results require that the entire routing space be thoroughly checked. Specifically, if $d>1$ happens at any time, we will set a $LEAK$ flag in the parent node to indicate that the children nodes are not able to cover the same routing space as the parent, which will lead to "missing" certain routing space to check for verfication. Therefore, in this case parent itself needs to be checked by the LPM rule. If there is not a child for a parent, we consider it as $d>1$. As long as there is one $LEAK$ flag initiated in a parent node, the flag will be carried over up to the nearest $REAL$ node, which can be the parent node itself. Once the process passes over a $REAL$ node, the flag will be cleared. Intuitively, we will check the forwarding equivalence over the rouing space covered by leaf nodes first, then over the remaining "leaking" one covered by internal nodes.    


\begin{figure}
	\begin{center}
		\includegraphics[width=.6\linewidth]{figures/BottomUpJointTrie}
		\caption{\label{fig:topdownjointtrie}Joint PATRICIA Trie After Bottom-Up Process}
	\end{center}
	\vspace{-8mm}
\end{figure}


\subsection{Algorithm}
\label{algorithm}

In the algorithm~\ref{alg:veritable} below, we show the pseudocode of our recursive function $VeriTable$ that quickly verifies whether the multiple forwarding tables are equivalent or not. If not, the corresponding LPM prefixes and next hops will be printed out. The algorithm consists of both the top-down next hops inheritance process and the bottom-up LPM matching and verification process. 

\begin{algorithm}
	\caption{Forwarding Equivalence Verification in the joint PT $T$. Depth-first post-order traversal over a PT. The initial values of $ancestor$ is $NULL$, and the initial value of $node$ is $T\rightarrow root$. We assume the root node of $T$ is a $REAL$ node.}\label{alg:veritable}
	\begin{algorithmic}[1]
		
		\Procedure{$VeriTable$}{$ancestor$, $node$}
		
		\If{$( node.type == REAL)$}
		\State $ancestor$ = $node$
		\EndIf
		
		\State l = $node\rightarrow l$
		\State r = $node\rightarrow r$
		
		\If{$( l \not=NULL)$}
			\If{$( l.type == REAL)$}
				\State $InheritNextHops(ancestor, l)$
			\EndIf
		\State $VeriTable(ancestor, l)$
		\EndIf
		
		\If{$( r\not=NULL)$}
			\If{$(r.type == REAL)$}
				\State $InheritNextHops(ancestor, r)$
			\EndIf
		\State $VeriTable(ancestor, r)$
		\EndIf
		
		\If{$(l == NULL) \land (r == NULL)$}
		\State {$CompareNextHops(node)$}
		\State \Return
		\EndIf
		
		\If{$( l \not=NULL) \land l.length - node.length > 1 $}
		\State $LeakFlag$ = 1
	
		\ElsIf{$( r \not=NULL) \land r.length - node.length > 1 $}
		\State $LeakFlag$ = 1
		
		\ElsIf{$(l \not=NULL \land r == NULL) \lor (r \not=NULL \land l == NULL)$}
		\State $LeakFlag$ = 1
		
		\ElsIf{$(l \not=NULL \land l.LeakFlag == 1) \lor (r \not=NULL \land r.LeakFlag == 1)$}
		\State $LeakFlag$ = 1
		\EndIf
		
		\If{$LeakFlag ==1 \land node.type == REAL$}
		\State {$CompareNextHops(node)$}
		\State $LeakFlag$ = 0
		\State \Return
		\EndIf
		
%		\If{$(LeftFlag \lor node\rightarrow l.length - node_{T}.length > 1  $\\$
%			\lor rFlag \lor  node_{T}.r.length - node_{T}.length > 1)$}
%		\If {$(node_{T}.glue)$}
%		\Return $True$
%		\Else \space $compareNextHops(node_{T})$
%		\State \Return $False$
%		\EndIf
%		\EndIf\\
%		\Return $False$
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%
\begin{algorithm}
	\caption{Inherit next hops from its nearest $REAL$ ancestor in the joint PT $T$}
	\label{alg:inherritnexthops}
	\begin{algorithmic}[1]
		\Procedure{$InheritNextHops$}{$ancestor$, $node$}
		\State AncestorNextHops = $ancestor \rightarrow NextHops$
		\State NodeNextHops = $node \rightarrow NextHops$
		\For{$i = 0...AncestorNextHops.length-1$}
			\If {$NodeNextHops[i]$ == -1} 
			\State $NodeNextHops[i]$ = $AncestorNextHops[i]$
			\EndIf
		\EndFor
%		\Do 
%		\State $nexthops_{T_{1..m}} = lookup(node_{T})$
%		\State $node_{T} = node_{T}.parent$
%		\doWhile {$nexthops_{T_{1..m}}.isNotFull$}
%		\If {$nexthops_{T_{1..m}}.areEqual$}
%		\Return $True$
%		\Else \space \Return $False$
%		\EndIf
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%
\begin{algorithm}
	\caption{Comparing next hops for a $node$. If there is a difference, print out all next hops on this node}
	\label{alg:comparenexthops}
	\begin{algorithmic}[1]
		\Procedure{$CompareNextHops$}{$node$}
		\State NodeNextHops = $node \rightarrow NextHops$
		\For{$i = 0...NodeNextHops.length-2$}
		\If {$NodeNextHops[i]$ != $NodeNextHops[i+1]$}
		\State Print prefix and all next hops of this node
		\State $break$
		\EndIf
		\EndFor
%		\Do 
%		\State $nexthops_{T_{1..m}} = lookup(node_{T})$
%		\State $node_{T} = node_{T}.parent$
%		\doWhile {$nexthops_{T_{1..m}}.isNotFull$}
%		\If {$nexthops_{T_{1..m}}.areEqual$}
%		\Return $True$
%		\Else \space \Return $False$
%		\EndIf
		\EndProcedure
	\end{algorithmic}
\end{algorithm}


%For the example that illustrates the algorithm we continue to use FIBs from Table \ref{tab:fibentry} as an example. The original and aggregated FIBs are shown on Figures \ref{fig:Merge}(a) and \ref{fig:Merge}(b).
%The trie of ``Version-II" Joint FIB is given on the Figure \ref{fig:Merge}. The LMPs in $T$ are the nodes $E, H, D, AF$. For each of these node, the algorithm will lookup for corresponding next hops from the original and aggregated FIBs and compare its values.

\subsection{An Example}
\label{algorithm}

\subsection{Proofs}
\label{proofs}

\section{The equivalence of forwarding tables problem}
\label{sec:bg}
We begin to consider the problem of the equivalence of forwarding tables by giving the formal definitions.
\begin{defn}Suppose there is a forwarding table $T$, which consists of entries $p^{1}, p^{2}, .., p^{n}$, where $p^{i} = \{0, 1\}^{l_{i}}$, where $l_{i}$ is the length of the entry $p^{i}, {i}\leq{n}$. Also there is a string $s = \{0, 1\}^{l_{s}}$. We can denote $p^{i}$ as $p_{1}p_{2}..p_{l_{i}}$ and $s$ as $s_{1}s_{2}..s_{l_{s}}$.
	\\ Then, $p^{i}$ is a \textbf{\textit{Longest Prefix Match}} for $s$ in $T$ (or $p^{i} = LPM_{s}(T)$), if
	\begin{enumerate}
		\item $l_{i} \leq l_{s}$
		\item $p^{i}$ is a Prefix for $s$ (or $p_{1} = s_{1}, p_{2} = s_{2}, .. , p_{l_{i}} = s_{l_{i}}$).
		\item $\nexists p^{j} = \{0, 1\}^{l_{j}}: p^{j}$ is a Prefix for $s$ and $l_{j} > l_{i}$.
	\end{enumerate}
\end{defn}
In the following definitions we denote the value of next hop for a prefix $p$ in the table $T$ as $nexthop(p)$.
\begin{defn}The forwarding tables $T_{1}, T_{2}, ..., T_{m}$ are \textbf{\textit{equivalent}}, if and only if, for every possible IP address $\omega = \{0,1\}^{n}$,  $nexthop(LPM_{\omega}(T_{1})) = nexthop(LPM_{\omega}(T_{2}))= ... = nexthop(LPM_{\omega}(T_{m}))$. $n$ is the fixed length of the IP address.
\end{defn}
According the definition above, to verify the equivalence of forwarding tables requires $2^{32}$ or $2^{128}$ depending on the format of forwarding tables (IPv4 of IPv6).  Our goal is to draw an equivalent definition with a feasible number of the required steps. To do that, we prove the property of the \textit{Joint Forwarding Table}, combined by entries of the comparable tables.
\begin{theorem}
		Let $T$ be a union of two routing tables $T_{1}, T_{2}, ..., T_{m}$. Then, $\forall \omega = \{0,1\}^{n}, LPM_{\omega}(T_{i}) = LPM_{p}(T_{i})$, where $p = LPM_{\omega}(T)$ and $i = 1, 2, ..., m$.
		\begin{proof}
			Let's denote entry $p$ as $p_{1}p_{2}..p_{l}$, its length $l\leq n$ and $\omega$ as $\omega_{1}\omega_{2}..\omega_{n}$. If $p = LPM_{\omega}(T)$, then $\omega = p_{1}p_{2}...p_{l}\omega_{l}\omega_{l+1}..\omega_{n}$. 
			\\ Suppose, $LPM_{p_{1}p_{2}...p_{l}\omega_{l}\omega_{l+1}..\omega_{n}}(T_{i}) \neq LPM_{p_{1}p_{2}..p_{l}}(T_{i})$. It is possible only if there is an entry $p^{'}$ in the routing table  $T_{i}$ such as its length $l < l^{'} \leq n$, and that entry is a Prefix for $w$. But then, that entry exists in $T$ and $p$ cannot be a \textbf{Longest Prefix Match} for $\omega$ and $T$. Thus there is a contradiction with the hypotheses of the theorem that $p = LPM_{\omega}(T)$.
		\end{proof}
\end{theorem} 
Let's then rewrite the Definition 2 according to the Theorem 1.
\begin{defn}The forwarding tables $T_{1}, T_{2}, ..., T_{m}$ are \textbf{\textit{equivalent}}, if and only if, $\forall \omega = \{0,1\}^{n}$,  $\forall p = LPM_{\omega}(T),$ where $T$ is the union of $T_{1}, T_{2}, ..., T_{m}, nexthop(LPM_{p}(T_{1})) = nexthop(LPM_{p}(T_{2}))$. 
\end{defn}
Although the new definition still refers the scope of IP addresses $\omega$, the set of \textit{Longest Prefix Matches} in $T$ is bounded by the number of entries in $T$ and can be defined regardless to $\omega$. We discuss it in the next section.


==> bg.tex_old.tex <==
\section{The equivalence of forwarding tables problem}
\label{sec:bg}
We begin to consider the problem of the equivalence of forwarding tables by giving the formal definitions.
\begin{defn}Suppose there is a forwarding table $T$, which consists of entries $p^{1}, p^{2}, .., p^{n}$, where $p^{i} = \{0, 1\}^{l_{i}}$, where $l_{i}$ is the length of the entry $p^{i}, {i}\leq{n}$. Also there is a string $s = \{0, 1\}^{l_{s}}$. We can denote $p^{i}$ as $p_{1}p_{2}..p_{l_{i}}$ and $s$ as $s_{1}s_{2}..s_{l_{s}}$.
	\\ Then, $p^{i}$ is a \textbf{\textit{Longest Prefix Match}} for $s$ in $T$ (or $p^{i} = LPM_{s}(T)$), if
	\begin{enumerate}
		\item $l_{i} \leq l_{s}$
		\item $p^{i}$ is a Prefix for $s$ (or $p_{1} = s_{1}, p_{2} = s_{2}, .. , p_{l_{i}} = s_{l_{i}}$).
		\item $\nexists p^{j} = \{0, 1\}^{l_{j}}: p^{j}$ is a Prefix for $s$ and $l_{j} > l_{i}$.
	\end{enumerate}
\end{defn}
In the following definitions we denote the value of next hop for a prefix $p$ in the table $T$ as $nexthop_{T}(p)$.
\begin{defn}The forwarding tables $T_{1}, T_{2}, ..., T_{m}$ are \textbf{\textit{equivalent}}, if and only if, for every possible IP address $\omega = \{0,1\}^{n}$,  $nexthop_{T_{1}}(LPM_{\omega}(T_{1})) = nexthop_{T_{2}}(LPM_{\omega}(T_{2}))= ... = nexthop_{T_{m}}(LPM_{\omega}(T_{m}))$. $n$ is the fixed length of the IP address.
\end{defn}
According the definition above, to verify the equivalence of forwarding tables requires $2^{32}$ or $2^{128}$ depending on the format of forwarding tables (IPv4 of IPv6).  Our goal is to draw an equivalent definition with a feasible number of the required steps. To do that, we prove the property of the \textit{Joint Forwarding Table}, combined by entries of the comparable tables.
\begin{theorem}
		Let $T$ be a union of two routing tables $T_{1}, T_{2}, ..., T_{m}$. Then, $\forall \omega = \{0,1\}^{n}, LPM_{\omega}(T_{i}) = LPM_{p}(T_{i})$, where $p = LPM_{\omega}(T)$ and $i = 1, 2, ..., m$.
		\begin{proof}
			Let's denote entry $p$ as $p_{1}p_{2}..p_{l}$, its length $l\leq n$ and $\omega$ as $\omega_{1}\omega_{2}..\omega_{n}$. If $p = LPM_{\omega}(T)$, then $\omega = p_{1}p_{2}...p_{l}\omega_{l}\omega_{l+1}..\omega_{n}$. 
			\\ Suppose, $LPM_{p_{1}p_{2}...p_{l}\omega_{l}\omega_{l+1}..\omega_{n}}(T_{i}) \neq LPM_{p_{1}p_{2}..p_{l}}(T_{i})$. It is possible only if there is an entry $p^{'}$ in the routing table  $T_{i}$ such as its length $l < l^{'} \leq n$, and that entry is a Prefix for $w$. But then, that entry exists in $T$ and $p$ cannot be a \textbf{Longest Prefix Match} for $\omega$ and $T$. Thus there is a contradiction with the hypotheses of the theorem that $p = LPM_{\omega}(T)$.
		\end{proof}
\end{theorem} 
Let's then rewrite the Definition 2 according to the Theorem 1.
\begin{defn}The forwarding tables $T_{1}, T_{2}, ..., T_{m}$ are \textbf{\textit{equivalent}}, if and only if, $\forall \omega = \{0,1\}^{n}$,  $\forall p = LPM_{\omega}(T),$ where $T$ is the union of $T_{1}, T_{2}, ..., T_{m}, nexthop_{T_{1}}(LPM_{p}(T_{1})) = nexthop_{T_{2}}(LPM_{p}(T_{2})) = ... = nexthop_{T_{m}}(LPM_{p}(T_{m}))$. 
\end{defn}
Although the new definition still refers the scope of IP addresses $\omega$, the set of \textit{Longest Prefix Matches} in $T$ is bounded by the number of entries in $T$ and can be defined regardless to $\omega$. We discuss it in the next section.


==> intro.tex_old.tex <==
\section{Introduction}
\label{sec:intro}
The Internet architecture divides the global network into Autonomous Systems (ASes). Every AS is assigned with unique Autonomous System Number (ASN), and a block of IP addresses - IP prefixes. For example, the IP prefix 92.65.64.0/24 represents the block of $2^{8}$ IP addresses with first 3 octets equal to 92, 65 and 64. The assignment of IP blocks and ASNs is regulated by Internet Assigned Numbers Authority (IANA). The routing within ASes is handled by Interior Gateway Protocols, such as OSPF or RIP. For inter-routing between different ASes, the mostly practised protocol is Border Gateway Protocol (BGP). 

BGP protocol implies sessions between a border AS router and its peers from other ASes. During BGP session, each AS announces to its peers its own prefixes, plus the routes to other IP prefixes on the network, learned from the other peers. The router running BGP accepts and announces the routes according to BGP policy set by AS administrator. BGP policy also qualifies the decision process on the best route among multiple routes to the same prefix. Once the choice is made, the best route is installed in the Forwarding Information Base (FIB) on the forwarding plane of the router. 

Forwarding Tables - or Forwarding Information Bases (FIBs) - consist of IP prefixes and corresponding next hops. On IP packet arrival, network router uses its forwarding engine to do a lookup into FIB to find the matching prefix for packet's destination IP address and then to forward the packet to the corresponding next hop. In case if there are multiple prefixes matching the same destination IP address, the one with the most number of bits is selected. This prefix is called a ``Longest Prefix Match" (LPM) for the matched IP address. 

The LPM lookup is a potential bottleneck. To avoid queuing delays contemporary routing engines run lookups at the line speed. The constant time lookup is performed at the price of the sophisticated hardware chips called ``Ternary Content Addressable Memory" (TCAM). The entries in FIB are sorted from more to less specific prefixes. Parallel TCAM lookup matches IP address to each entry in FIB, so the top matched entry will be the LPM. 

Different factors, such as the growth of the Internet, traffic engineering and multi-homing add to the superlinear growth of the number of separately announced prefixes. This became a serious concern for network operators working in the Default-Free Zone (DFZ).  Because every TCAM has the limitation on FIB size it can store, the DFZ operators have to upgrade the expensive hardware by analogs with bigger capacities. In addition, hardware-implemented parallel search in TCAM is highly energy-consumptive  and needs more cooling facilities.

\begin{table}[tbp]
	\centering
	\small
	\caption{FIB aggregation process}
	\captionsetup{justification=centering}
	\label{tab:fibentry}
	%	\vspace{0mm}
	\subfloat[Original FIB table]{
		\begin{tabular}{| c | c | c | }
			\hline
			Label & Prefix  & Next hop   \\ \hline
			A & 92.65.0.0/15 & 1    \\ \hline
			B & 92.65.128.0/17 & 1    \\ \hline
			C & 92.65.0.0/17 & 2    \\ \hline
			D & 92.65.64.0 /18 & 3    \\ \hline
			E & 92.65.0.0/19 & 3    \\ \hline
		\end{tabular}
		\label{tab:originalfibentry}
	}
	\\
	\subfloat[Compressed FIB table]{
		\begin{tabular}{| c | c | c | }
			
			\hline
			Label & Prefix  & Next hop   \\ \hline
			F & 92.65.0.0/15 & 1    \\ \hline
			G & 92.65.0.0/17 & 3    \\ \hline
			H & 92.65.32.0/19 & 2    \\ \hline
		\end{tabular}
		\label{tab:filteredfibentry}
	}
	\vspace{-3mm}
\end{table}

Finding solution for routing table scalability problem is particularly important in the context of coming IPv6 era (with address space approximately equal to  $3.4*10^{38}$ possible values).
The long-term solution is to review current network protocols and network architecture. Zhao et al.~\cite{zhao2010routing} describe possible revision of the networking business model in order to compensate expenses of DFZ-operators on upgrading their network operational resources. However, the deployment of such solutions is difficult as it can not be done locally within one AS.

In contrast, FIB compression does not require neither the global deployment nor the operational or hardware expenses. Analysis of the global (FIB\cite{meng2005ipv4},\cite{cidr_report}) shows that about 50\% of BGP-announced prefixes represent the sub-blocks of IP address space, that is also advertised by BGP. Some of this overlapping prefixes may (and most likely) share the same next hop (the number of possible next hops depends on the number of peers that AS has). The most obvious compression can be achieved by eliminating entries with prefixes overlapped by more specific prefixes present in FIB and having the same next hop. On the other hand, entries with more specific prefixes can be eliminated if they share the same next hop with less specific prefixes entries. The examples of such algorithms are Level-1 and Level-2 aggregation.  Algorithms as ORTC~\cite{draves1999constructing} or ORTC-based FIFA~\cite{liu2013fifa} use more sophisticated compression techniques and may reduce FIB by up to 70\%. An example of the original and FIFA-compressed FIB is given on the Table \ref{tab:fibentry}.

Any compression approach must efficiently handle constant next hop updates and prefix removals. The number of such announcements can reach tens of thousand per second during spikes.

We say that the compressed FIB is equivalent to the original FIB, if applying compressed FIB to the router doesn't change router's forwarding behavior: a packet with any possible IP address is forwarded to the same next hop as before FIB compression. Establishing of the equivalence between FIBs is a practical way to avoid misbehavior of the forwarding engine and debug new FIB compression techniques. Given the number of possible 32-bit and 128-bit IP addresses ($2^{32}$ for IPv4  and $2^{128}$ for IPv6 addresses), the brute-force verification of the forwarding equivalence between tables is not realistic.   

\begin{figure}
	\begin{center}
		\includegraphics[clip = true, trim = 2cm 5cm 5cm 1cm, width=.3\linewidth, width=0.4\textwidth]{figures/IMG_TaCo_normalized}
		\caption{\label{fig:taco}Leaf-pushed binary tree for FIB (Table \ref{tab:originalfibentry})}
	\end{center}
	\vspace{-8mm}
\end{figure} 

 % if we have T_1...T_n than we need to run first T_1/T_2 comparison. 2 traversals per each tree. Then if we compare T_2 and T_3, we need to run an additional traversal for T_2 to compare it with T_3. Thus every tree except the first and the last (2 traversals per each tree) one will have to run 3 traversals. 3(n - 2) + 2 + 2 = 3n - 2. 

In this work we present the FIB equivalence verification algorithm with the minimized number of lookups and memory accesses required to run for verifying the equivalence of two or more FIBs. The output of algorithm is either the equivalence statement, or the scopes of IP addresses that will be forwarded differently in the comparable FIBs. We begin with giving the mathematical definition to the problem in Section~\ref{sec:bg}. There, we prove the crucial property of the set of all LPMs of the joint FIB $T$, constructed by adding the entries of the comparable FIBs $T_{1}, T_{2}, ... , T_{n}$ and removing the duplicate entries. The property allows to use the entries of the set of $LPM(T)$ instead of IP addresses, for running next hop comparisons in tables $T_{1}, T_{2}, ... , T_{n}$.

In Section~\ref{sec:design} , we show the implementation of the algorithm based on the properties we proved in the previous section. In the Section~ \ref{sec:evaluation} , we evaluate the algorithm by applying it to the real-world IPv4 and IPv6 routing data from RouteViews Project. In  Section~\ref{sec:related} we discuss the other approaches to solve the FIB equivalence verification problem. In Section~\ref{sec:conclusion} we draw the conclusions on this paper and discuss the possible application of the algorithm and our further steps.

%\begin{figure}
%	\centering
%	\includegraphics
%	\caption{Autonomous Systems and Global Network}
%\end{figure}

==> related.tex <==
\section{Related Work}
\label{sec:related1}
Related

==> simulation.tex <==
\section{Emulating an ISP network}
\label{sec:simulation}

The second objective of our work is to set up a \emph{realistic network environment} to demonstrate the performance of our FIB aggregation algorithm.  To this end, we use VirtualBox, BGPSimple, and real ISPs' routing data to emulate a real operational network.  Note that our methodology can be used to emulate any network, but in this section, we use the Internet2 Abilene topology as an example to illustrate our methodology.  

\begin{figure}[tb]
\begin{center}
     \includegraphics[width=2.5in]{figures/topology}
\caption{\label{fig:topology}Virtual Network Setup}
\end{center}
\vspace{-8mm}
\end{figure}

Figure~\ref{fig:topology} shows our virtual network, which includes a total of 9 routers in the Internet2 topology and 9 external BGP speakers belonging to other ISPs that exchange routing information with Internet2.  Each node is on a separate virtual machine.    Each Internet2 router runs either the original Quagga or our updated version of Quagga (specifically the Zebra, OSPF, and BGP daemons).  Each BGP speaker runs the BGPSimple program that sends real routing updates to the BGP peer. 

%TODO: do we run OSPFN on the BGP speaker nodes?
We use OSPF to establish intra-domain connectivity among all of the Internet2 nodes.
%which results in route additions to the Kernel FIB for complete intra-domain connectivity. 
The BGP daemons on each Internet2 node then use this base connectivity to establish BGP peering session with their iBGP peers.  For  simplicity, we use full-mesh iBGP peering, i.e., every router has an iBGP session with every other router in the same network.  For a larger topology, we can use Route Reflectors to reduce the number of iBGP sessions.

In order to attain equivalence between the virtual network and a real world ISP, we need the presence of the huge volume of BGP routing updates in the Internet.  Fortunately, BGP routing table and updates from many ISPs are being collected by a number of projects.  
%This is done through tabledump and update �les which are organized chronologically for a lot of actual internet router pre�xes. These �les include snapshots of routing tables of BGP routers in the internet formatted in the form of route announcements and withdrawals. 
We use the BGP data from the RouterViews project of the University of Oregon~\cite{routeviews} and the BGPMon project of Colorado State University~\cite{BGPmon}. The RouterViews project provides BGP table dumps and update files archived at regular intervals while the BGPMon project provides \emph{live} BGP updates in addition to archived BGP data. 
%These are two among the many freely available data sources which make BGP routing information available and it is possible to use these �les as feeds for BGP speaker applications.

%A real-world routing network transits frequent and consistent volume of network control traf�c in order to maintain end-to-end connectivity between its nodes. The control updates format and handshake mechanisms vary depending on the routing protocol being followed. But these updates, although not constituting the majority of the network traf�c, form a signi�cant part as they control the forwarding information held in the routing tables and thereby the overall routing process. The next section details how we add real-world routing updates to our experimental setup.

%We can make a virtual network equivalent to a real-world routing architecture if we need to simulate a very similar level of control traffic. This requires the infusion and propagation of an equivalent volume of protocol speci�c updates which get processed by the individual routing nodes and cause updates to the routing tables. For the purpose of this paper and our research we will focus the control traf�c speci�c to only the BGP protocol. 

We modified the BGPSimple program to pump the BGP data into the network.  The program first reads a routing table from a BGP table dump file (from RouteViews or BGPMon) and then sends the resulting BGP updates over its BGP session so that the peer can establish an initial BGP table.  Since there are hundreds of thousands of entries in a full routing table, we added pacing to the BGPSimple program  so that the peer does not become overwhelmed by the initial influx of updates.  The program then sends subsequent BGP updates as they become available.  These updates are obtained from either the BGP update files downloaded from RouteViews or a live stream of BGP updates from BGPMon.  
%The BGP speaker can also filter BGP updates based on many parameters such as originating peer and address prefix being advertised. 
%These updates are spoken in the form of BGP announcements and withdrawals which when reach the connected routers, are processed and propagated to other BGP peers in the network. In other words, the BGP feed provided to the speaker in a way determine the control traffic moving around in the network. Therefore to make a node on our virtual network function in a similar to an actual BGP router only required feeding routing updates as processed by latter.
In order to evaluate the performance of our system under high routing load, we used large routing tables with 450,000 prefixes on average. 
%The speakers were also configured to switch over to live BGP update channel of Colorado State once they finish processing their initial tabledump files.



%As each node of the Abilene network represents a separate BGP router having its own volume of peering update channel, we added a total of 9 BGP Speaker nodes (ones speaker for each virtual router node) to our setup. Each of these speakers were con�gured for processing a BGP tabledump �le collected for a recent date from the data sources corresponding to an actual internet BGP router. 
